Numerical Study of the Two-Species Vlasov-Amp\`{e}re System: Energy-Conserving Schemes and the Current-Driven Ion-Acoustic Instability

In this paper, we propose energy-conserving Eulerian solvers for the two-species Vlasov-Amp\`{e}re (VA) system and apply the methods to simulate current-driven ion-acoustic instability. The algorithm is generalized from our previous work for the single-species VA system and Vlasov-Maxwell (VM) system. The main feature of the schemes is their ability to preserve the total particle number and total energy on the fully discrete level regardless of mesh size. Those are desired properties of numerical schemes especially for long time simulations with under-resolved mesh. The conservation is realized by explicit and implicit energy-conserving temporal discretizations, and the discontinuous Galerkin (DG) spatial discretizations. We benchmarked our algorithms on a test example to check the one-species limit, and the current-driven ion-acoustic instability. To simulate the current-driven ion-acoustic instability, a slight modification for the implicit method is necessary to fully decouple the split equations. This is achieved by a Gauss-Seidel type iteration technique. Numerical results verified the conservation and performance of our methods.

==> numerical-badpaper.tex <==
\subsection{numerical-bad paper}
\begin{figure}[!htbp]
%
 \subfigure[Electron. Total particle number.]{\includegraphics[width=0.45\textwidth]{mass1case1.eps}}
 \subfigure[Ion, Total particle number.]{\includegraphics[width=0.45\textwidth]{mass2case1.eps}}\\
  \subfigure[Electron. Momentum]{\includegraphics[width=0.45\textwidth ]{mom1case1.eps}}
 \subfigure[Ion. Momentum]{\includegraphics[width=0.45\textwidth ]{mom2case1.eps}}\\
  %\subfigure[Bump-on-tail instability. Total particle number.]{\includegraphics[width=0.45\textwidth ]{bumpcharge.png}}
% \subfigure[Bump-on-tail instability. Total energy.]{\includegraphics[width=0.45\textwidth ]{bumpenergy1.eps}}
\caption{Error evolution. Case 1. $CFL = 20$. $50\times100$ mesh. Time scale: $\bar{t}=2.38\,ns$}
%\label{figure_energy1}
\end{figure}
\begin{figure}[!htbp]
%
 \subfigure[Electron. Kinetic Energy]{\includegraphics[width=0.45\textwidth]{kinetic1case1.eps}}
 \subfigure[Ion, Kinetic Energy]{\includegraphics[width=0.45\textwidth]{kinetic2case1.eps}}\\
  \subfigure[Electric Energy]{\includegraphics[width=0.45\textwidth ]{electriccase1.eps}}
 \subfigure[Total Energy]{\includegraphics[width=0.45\textwidth ]{totalecase1.eps}}\\
  %\subfigure[Bump-on-tail instability. Total particle number.]{\includegraphics[width=0.45\textwidth ]{bumpcharge.png}}
% \subfigure[Bump-on-tail instability. Total energy.]{\includegraphics[width=0.45\textwidth ]{bumpenergy1.eps}}
\caption{Error evolution. Case 1. $CFL = 20$. $50\times100$ mesh. Time scale: $\bar{t}=2.38\,ns$}
%\label{figure_energy1}
\end{figure}
\begin{figure}[!htbp]
%
 \subfigure[Electron. ]{\includegraphics[width=0.45\textwidth]{density1case1.eps}}
 \subfigure[Ion.]{\includegraphics[width=0.45\textwidth]{density2case1.eps}}\\
%  \subfigure[Electric Energy]{\includegraphics[width=0.45\textwidth ]{electriccase1.eps}}
% \subfigure[Total Energy]{\includegraphics[width=0.45\textwidth ]{totalecase1.eps}}\\
  %\subfigure[Bump-on-tail instability. Total particle number.]{\includegraphics[width=0.45\textwidth ]{bumpcharge.png}}
% \subfigure[Bump-on-tail instability. Total energy.]{\includegraphics[width=0.45\textwidth ]{bumpenergy1.eps}}
\caption{Density (maximum). Case 1. $CFL = 20$. $50\times100$ mesh. Time scale: $\bar{t}=2.38\,ns$}
%\label{figure_energy1}
\end{figure}


==> shavafig.tex <==
%%
%% April 18, 2001
%%
%% shavafig.sty
%%
%% DESCRIPTION:
%%   \centerfig[OPT]{FILENAME}{CAPTION} centers a eps figure.  The label for
%%       the figure will be FILENAME.
%%
%%     OPT is a spec string argument to epsfig.  E.g. width=4in, height=5in.
%%         Note that OPT will overide the default spec string 
%%         'height=3.65in'
%%
%%     FILENAME is the name of the eps file without the .eps.  Default is to
%%     look for the figure in the current directory unless it has been reset
%%     with \setfiguredirectory.
%%     
%%     CAPTION is the caption for the figure
%%
%%   \setcenterfigwidth{WIDTH} sets the default spec string to 'width=WIDTH'
%%
%%   \setcenterfigheight{HEIGHT} sets the default spec string to 'height=HEIGHT'
%%
%%   \resetcenterfig sets default spec string to 'height=3.65in'
%%
%% INSTALLATION:
%%   Put this file where your TeX looks for inputs.
%%
%% DOCUMENTATION:
%%  See centerfig.tex, which might be appended to this file.
%%
%% CODE:
%
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{rotating}
\RequirePackage{subfigure}

\ProvidesPackage{shavafig}

% Globals
\newlength{\@def@fig@scalar}
\setlength{\@def@fig@scalar}{3.65in}
\newlength{\@fig@scalar}
\setlength{\@fig@scalar}{\@def@fig@scalar}
\newcommand{\@fig@spec}{height}
\newcommand{\@fig@dir}{.}

% Functions

\newcommand{\setfiguredirectory}[1]
{
  \renewcommand{\@fig@dir}{#1}
}

\newcommand{\centerfig}[4][\@fig@spec=\@fig@scalar] 
{ 
  \begin{figure}[htbp]
  \begin{center}
  \epsfig{file=\@fig@dir/#2.eps,#1}
  \caption[#4]{\label{#2}#3}
  \end{center}
  \end{figure}
}

\newcommand{\pairfig}[4]
{ 
  \begin{figure}[htbp]
  \begin{center}
  \subfigure[]{\epsfig{file=\@fig@dir/#1.eps,height={.38\textheight}}} \\
  \subfigure[]{\epsfig{file=\@fig@dir/#2.eps,height={.38\textheight}}} \\
  \caption[#4]{\label{#1}\label{#4}#3}
  \end{center}
  \end{figure}
}

\newcommand{\quadfig}[6][\@fig@spec=\@fig@scalar]
{ 
  \begin{figure}[htbp]
  \begin{center}
  \subfigure[]{\epsfig{file=\@fig@dir/#2.eps,width={.48\textwidth}}} 
  \subfigure[]{\epsfig{file=\@fig@dir/#3.eps,width={.48\textwidth}}} \\
  \subfigure[]{\epsfig{file=\@fig@dir/#4.eps,width={.48\textwidth}}} 
  \subfigure[]{\epsfig{file=\@fig@dir/#5.eps,width={.48\textwidth}}} \\
  \caption{\label{#2}\label{#3}#6}
  \end{center}
  \end{figure}
}


\newcommand{\landscapefig}[4][width=\textheight]
{ 
  \begin{sidewaysfigure}[htbp]
  \centering
  \epsfig{file=\@fig@dir/#2.eps,#1}
  \caption[#4]{\label{#2}#3}
  \end{sidewaysfigure}
}

\newcommand{\setcenterfigheight}[1]
{ 
  \renewcommand{\@fig@spec}{height}
  \setlength{\@fig@scalar}{#1}
}

\newcommand{\setcenterfigwidth}[1]
{ 
  \renewcommand{\@fig@spec}{width}
  \setlength{\@fig@scalar}{#1}
}

\newcommand{\resetcenterfig}
{ 
  \renewcommand{\@fig@spec}{height}
  \setlength{\@fig@scalar}{\@def@fig@scalar}
}


